Turbo: Effective Caching in Differentially-Private Databases

Differentially-private (DP) databases allow for privacy-preserving analytics over sensitive datasets or data streams. In these systems, user privacy is a limited resource that must be conserved with each query. We propose Turbo, a novel, state-of-the-art caching layer for linear query workloads over DP databases. Turbo builds upon private multiplicative weights (PMW), a DP mechanism that is powerful in theory but ineffective in practice, and transforms it into a highly-effective caching mechanism, PMW-Bypass, that uses prior query results obtained through an external DP mechanism to train a PMW to answer arbitrary future linear queries accurately and "for free" from a privacy perspective. Our experiments on public Covid19 and CitiBike datasets show that Turbo with PMW-Bypass conserves 1.7-15.9x more budget compared to vanilla PMW and simpler cache designs, a significant improvement. Moreover, Turbo provides support for range query workloads, such as timeseries or streams, where opportunities exist to further conserve privacy budget through DP parallel composition and warm-starting of PMW state. Our work provides a theoretical foundation and general system design for effective caching in DP databases.

==> Makefile <==
PAPER=dp-caching
LATEX=pdflatex

BIBTEX=bibtex

SRCS=$(PAPER).tex $(wildcard sections/*.tex) $(wildcard sections/*/*.tex)
REFS=$(wildcard bib/*.bib)
FIGS=$(wildcard figures/*)
STYLE=$(wildcard style/*)

.PHONY: results $(PAPER).pdf clean

all: results $(PAPER).pdf

results:
	+make -C $@

$(PAPER).pdf: $(SRCS) $(REFS) $(FIGS) $(STYLE)
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)


submission: $(PAPER).pdf
	cp $(PAPER).pdf submission/

split: $(PAPER).pdf
	pdftk $(PAPER).pdf cat 1-16 output turbo_main.pdf
	pdftk $(PAPER).pdf cat 17-25 output turbo_appendix.pdf

clean:
	rm -f *.dvi *.aux *.log *.blg *.bbl \
          $(PAPER).ps $(PAPER).pdf \
          $(PAPER)-single.pdf $(PAPER)-single.ps


==> results/Makefile <==
FIGS = \
	monoblock/covid19/laplace_vs_hybrid/cumulative_budget_utilization \
	monoblock/covid19/heuristics/cumulative_budget_utilization \
	monoblock/covid19/learning_rates/cumulative_budget_utilization \
	monoblock/covid19/convergence/lr_convergence \
	monoblock/citibike/laplace_vs_hybrid/cumulative_budget_utilization \
	multiblock/static/covid19/laplace_vs_hybrid/cumulative_budget_utilization \
	multiblock/streaming/covid19/laplace_vs_hybrid/cumulative_budget_utilization \
	multiblock/streaming/citibike/laplace_vs_hybrid/cumulative_budget_utilization \
	multiblock/static/covid19/laplace_vs_hybrid/cumulative_budget_utilization \
	multiblock/static/citibike/laplace_vs_hybrid/cumulative_budget_utilization \
	multiblock/static/covid19/tree/tree_vs_linear \
	multiblock/static/covid19/tree/tree_vs_linear_zipf1 \
	multiblock/streaming/syseval/runtime \
	monoblock/syseval/runtime \
	monoblock/covid19/heuristics2/budget_utilization_zipf1 \
	monoblock/covid19/heuristics2/budget_utilization_zipf1_5 \



GNUPLOT := gnuplot
EPS2PDF := epstopdf
EPS2PNG := convert
PDFFILES = $(FIGS:=.pdf)
PNGFILES = $(FIGS:=.png)

all: $(PDFFILES) Makefile

pngs: $(PNGFILES)

list:
	@echo $(PDFFILES) $(PNGFILES)

%.pdf: %.eps
	$(EPS2PDF) $< --outfile $@.tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/screen -dCompressFonts=true -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -f $@.tmp.pdf
	rm $@.tmp.pdf

%.png: %.eps
	$(EPS2PNG) $< -background white -alpha remove -alpha off -rotate 90 $@

%.eps: %.plot %.csv boilerplate* Makefile
	$(GNUPLOT) -e "set terminal postscript eps enhanced monochrome; set output \"$@\"" $<

clean:
	@rm -f $(PDFFILES) $(PNGFILES)


==> sections/design/disaggregated-pmws.tex <==
\subsection{\Disaggregatedpmw}
\label{sec:disaggregated-tree-of-pmwsbypasses}

\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/disaggregated-tree-of-pmw-bypasses}
    \caption{\small {\bf How the \disaggregatedpmw works for the example in \F\ref{fig:example-tree-of-pmw-bypasses}.}
    }
    \label{fig:disaggregated-tree-of-pmwbypasses}
\end{figure}

\xxx{TODO(students)}

Figure~\ref{fig:disaggregated-tree-of-pmwbypasses} illustrates the core functionality of our \disaggregatedpmw, while \A\ref{alg:disaggregated-pmw} shows the more specific algorithm.

\begin{algorithm}[ht]
    \centering
    \begin{algorithmic}[1]
        \State \pierre{Very temporary draft, please ignore for now!}
        \While{$\textproc{PrivacyAccountant.HasBudget()}$}
        \State Receive next query $q$
        \State $Nodes \gets \textproc{SplitQuery}(q)$
        \For{$i \in Nodes$}
        \If{$\textproc{Heuristic.IsHistogramReady}(h_i,q_i, \alpha_i, \beta_i)$}
        \State $r_i \gets q_i(h_i)$
        \Else{}
        \State $r_i \gets \lap{1/\epsilon_i n_i}$
        \EndIf
        \State $r_{hist} = \textproc{Agg}(r_i)$
        \If{$\textproc{SVCheck}(r_{hist}, q, \alpha_{SV}, \beta_{SV})$}
        \State Recompute with Laplace
        \State $r_{hist} = \textproc{Agg}(r_i)$
        \EndIf
        \State Output $R = \textproc{Agg}(r_{hist}, r_{lap})$
        \EndFor
        \EndWhile
    \end{algorithmic}
    \caption{\bf \disaggregatedpmw algorithm.}
    \label{alg:disaggregated-pmw}
\end{algorithm}

\heading{SV Accounting.}
For simplicity, \A\ref{alg:disaggregated-pmw} uses one sparse vector per requested window.
For $T$ blocks, there are $T-\ell + 1$ such windows of length $\ell$. This represents $O(T\cdot T_{\max})$ sparse vectors if queries demand less than $T_{\max}$ blocks.

Alternatively, we can group similar queries under a single sparse vector.
More precisely, each request $[i, i+\ell)$ of length $2^{k-2} < \ell \le 2^{k-1}$ is assigned to a sparse vector covering $2^k$ blocks $[q2^{k-1}, q2^{k-1} + 2^k)$ with $q = \lfloor i / 2^{k-1} \rfloor$.
Indeed, for $i = q2^{k-1} + r$ with $q\in \mathbb{N}$ and $r \in [0, 2^{k-1})$ the query is properly covered since $i +\ell = q2^{k-1} + r + \ell < q2^{2k-1} + 2 \cdot 2^{k-1}$.
Each sparse vector now has to account for the sensitivity of the smallest request it covers, which contains at least $2^{k-2}$ blocks.
This represents only $O(T)$ sparse vectors if queries demand less than $T_{\max}$ blocks (two truncated binary trees of sparse vectors).

\heading{Guarantees.}

\begin{theorem} The \disaggregatedpmw preserves $\epsilon$-DP and is $(\alpha,\beta)$-accurate for each query it answers.
    \pierre{Unlike \treeofpmwbypasses, no limit on the number of blocks, but if queries request non-contiguous
        ranges we will run out of budget faster.}
\end{theorem}

\begin{theorem} Convergence -- if Pierre is able to prove something under the "partial synchrony"-like assumption.
\end{theorem}


==> sections/design/exact-match-cache.tex <==
\subsection{\exactcache}
\label{sec:exact-match-cache}

\iffalse
\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/PMW-Bypass-combined-with-exact-match-cache}
\caption{\small {\bf PMW-Bypass combined with an \exactcache via variance reduction.}  Uses variance reduction to reduce the amount of privacy budget used if the same query has been run before but with lower $\alpha$.
}
\label{fig:exact-cache}
\end{figure}
\fi

\todostudents{RFI: Will we have variance reduction evaluated?  Depending on this, this section will be written very differently, so pls let me know as soon as you have some info regarding that.}




==> sections/design/notation.tex <==
\subsection{Terms and Notation}
\label{sec:notation}

Describing our mechanisms in detail necessitates some notation, definitions, and simplifications, which we next introduce.


\heading{Linear queries.}




==> sections/evaluation.tex <==
% \section{Evaluation}
% \label{sec:evaluation}

% We evaluate \sysname in the three use cases described in \S\ref{sec:use-cases}, using two public timeseries datasets: \covid19 and \citibike.
% For each use case we answer the critical question: {\em Does \sysname significantly improve privacy budget consumption compared to reasonable baselines for each setting?}
% This corresponds to evaluating our design goals (G5) and (G6) in \S\ref{sec:goals}.
% In addition, each setting lets us evaluate a different set of caching mechanisms, answering different key questions about our design:

% %\begin{itemize}
% {\bf (1)} {\bf \Nonpartitioneddb:} \sysname is instantiated with a single \pmwbypass and \exactcache, letting us evaluate the \pmwbypass object, including its \empiricalconvergence and the impact of its heuristic and learning rate parameters.

%     {\bf (2)} {\bf \Partitionedstaticdb:} Since the datasets are timeseries, we assume data is partitioned by time (week-by-week) and most queries access different time windows.  We instantiate \sysname with the tree-structured \pmwbypass and \exactcache, letting us compare our tree-structured cache to a single \exactcache, and also to more powerful baselines for this setting, such as a \exactcachetree and a histogram-per-partition PMW.

%     {\bf (3)} {\bf \Partitionedstreamingdb:} \sysname is instantiated with the tree of \pmwbypasses and \exactcaches, but also with our histogram warm-up mechanisms.  Since new partitions arrive over time, after older partitions have already been queried, new histograms have an opportunity to be warm started.  This lets us evaluate the effectiveness of our two warm-up mechanisms.
% %\end{itemize}

% \vspace{0.2cm}
% Overall, our results show that \pmwbypass unleashes the power of \pmw, so far locked within an impractical theoretical construct, and significantly improves privacy budget consumption for linear queries over today's common practice of just having an exact-match cache (goal (G5)).
% Moreover, \sysname as a whole seamlessly applies to multiple settings, with its novel \pmwbypasstree structure proving especially effective in the case of timeseries and other workloads where range queries pervade, wherein the \sysname can leverage parallel composition (goal (G6)).
% We find \sysname is fairly easy to configure (goal (G7)) and can be tuned to optimize \empiricalconvergence -- rather than based on theoretical convergence as has been done in the past -- to make it even more effective in practice (goal (G4)).
% %With these results, we can finally confirm that \pmws {\em can} in fact be made to be useful in practice.  <-- this should appear in the intro/abstract.
% Finally, while our focus is on privacy budget usage, we also include a basic runtime and memory evaluation.  We find that for our datasets, \pmwbypass and \sysname can be made to scale through some engineering, and expect that further research will be needed to ready them for larger-domain data.

% \subsection{Methodology}
% \label{sec:evaluation:methodology}

% \begin{table}
%     \footnotesize
%     \centering
%     \begin{tabular}{|l|l|l|l|}
%         \hline
%                         & {\bf Dataset}       & {\bf Workload}       & {\bf Partitioning} \\
%         \hline
%         {\bf \covid19}  & Num. attributes: 4  & Query pool:          & Num. weeks: 50     \\
%                         & Dataset size $n=XX$ & \ \ \ \ 34,425       & Avg. rows/week:    \\
%                         & Domain size $N=128$ & $\kzipf \in \{0,1\}$ & \ \ \ \ XX         \\
%         \hline
%         {\bf \citibike} & Num. attributes: 8  & Query pool:          & Num. weeks: 50     \\
%                         & $n=XX$              & \ \ \ \ 2,485        & Avg. rows/week:    \\
%                         & $N=604,800$         & $\kzipf=0$           & \ \ \ \ XX         \\
%         \hline
%     \end{tabular}
%     \vspace{0.1cm}
%     \begin{tabular}{|l|l|l|}
%         \hline
%                          & {\bf Default values of parameters}        \\
%         \hline
%         {\bf Privacy}    & $\epsilon_G=10$, $\delta_G=0$             \\
%         \hline
%         {\bf Accuracy}   & $\alpha=0.05$, $\beta=0.001$              \\
%         \hline
%         {\bf Workload}   & \covid19 $\kzipf=1$, \citibike $\kzipf=0$ \\
%         \hline
%         {\bf \pmwbypass} & Heuristic: $C_0=100$, $S_0=5$             \\
%                          & External update: $\tau=XX$, $\gamma=XX$   \\
%                          & Learning rate: $\lr=0.2$                  \\
%         \hline
%     \end{tabular}
%     \vspace{0.35cm}
%     \caption{{\small {\bf Methodology.} Top: Dataset, workload, and partitioning characteristics of \covid19 and \citibike evaluations. Bottom: Default values for various parameters (assume these unless stated otherwise).}}
%     \label{tab:datasets}
% \end{table}

% For each dataset, we develop {\em query workloads} to use in our evaluation by first (1) creating a {\em pool} of linear queries and then (2) sampling as many queries as we need from this pool, according to a parameterized Zipfian distribution.
% The Zipfian distribution encodes the fact that certain queries may be more likely to be issued repeatedly than others, and has been previously used in traditional caching literature~\cite{ycsb,twitter-cache,atikoglu2012workload}.
% We detail the datasets and workload generation methodology next, after which we define the relevant metrics for evaluation.
% A key distinction between the \covid19 and \citibike methodologies is that the former uses a completely synthetic query pool, while the latter uses a query pool based on {\em real-user queries} from existing analyses people have done on \citibike.
% %We use the former as a {\em microbenchmark} that we can tune to analyze different settings.
% %We use the latter as a {\em macrobenchmark} to glean how \sysname might behave on real queries.

% \T\ref{tab:datasets} summarizes key details of our datasets, workloads, and partitioning characteristics (top), as well as values for various parameters we use in each use case (bottom).
% Unless otherwise stated, the reader can assume these default values.

% \heading{\covid19.} {\em Dataset:} We take a dataset of daily Covid-19 tests released by California between \xxx{XX and XX (dates)}. The original dataset consists of daily {\em aggregate information} -- number of Covid tests and their positivity -- for various demographic groups defined by age $\times$ gender $\times$ ethnicity.  By combining this dataset with US Census data~\cite{}, we generate a {\em synthetic dataset} containing \xxx{$n=XX$} per-person test records, each consisting of the date and four attributes: positivity, age, gender, and ethnicity.  Domain sizes of these attribute are 2, 2, 4, and 8, respectively, so the dataset's domain size is $N=128$.  The datasets spans $XX$ weeks at $XX$ records/week on average, hence in the partitioning use cases, we will have up to this many partitions.
%     {\em Query pool:} For this dataset, we create a synthetic and rich pool of correlated queries comprising all possible count queries that can be posed of the \covid19 dataset: specifically, all the 1-, 2-, 3-way marginals.
% This gives a total of $34,425$ unique queries, plenty for us to microbenchmark \sysname in different settings.

% \heading{\citibike.} {\em Dataset:} We take a dataset of New York City bike rentals released by the city between \xxx{XX and XX (dates)}.  It contains details of {\em individual rides}, including: start and end date and time, start and end geo-location, exact route taken, as well as the renter's gender and age.
% The original dataset contains very granular information (such as 4,000 distinct geo-locations and 100 ages), resulting in high-dimension data that is neither amenable to privacy-preserving analyses nor to PMWs, whose histograms are exponential in domain size.  Since all the real-user analyses we found consider the data at coarser granularity (such as broader locations and age brackets), we transform the dataset by grouping geo-locations into ten neighborhoods and ages into XX brackets.
% Our dataset has $n=XX$ records, domain size of $N=604,800$, and spans $XX$ weeks at $XX$ records/week on average.

%     {\em Query pool:} For this dataset, we seek a more ``plausible'' pool of queries instead of a purely synthetic one.  We gather a set of existing analyses created by various people and posted online for this dataset.  We specifically scour the Public Tableau Visual Analytics service~\cite{https://public.tableau.com/app/discover} for \citibike\ {\em workbooks}, which are interactive, visual analyses of a dataset (for example~\cite{tableau-link-for-a-story}).
% Based on XX workbooks, we derived 30 distinct queries, most of which contain `GROUP BY' statements that can be decomposed into multiple, individual {\em primitive queries} that interact with \sysname histograms.
% For \sysname, this results in a $2,485$-query pool, smaller than \covid19's, but the queries are real.
% We hence use it as a macrobenchmark.

% \heading{Workload generation.}
% We use different Zipfian distributions to explore effect of the skewness on the performance of the caches. %, which has implications to hitrates in, for example, exact-match caches.
% Given a pool of queries, we generate queries with a Poisson process where each new query is sampled independently from a Zipf distribution over the pool of queries.
% The PDF of the Zipf distribution is: $f_k(x)=\frac{1}{x^k \sum_{i=1}^{Q}(1/i)^k}$, where $Q>0$ is the number of queries generated for the workload and $k>0$ (denoted henceforth $\kzipf$) is the parameter of the Zipf distribution that controls its skewness.
% When $\kzipf=0$, queries are sampled uniformly at random; and when $\kzipf \to \infty$ the Poisson process always outputs the same query.
% We perform evaluation with a number of $\kzipf$ values, but include here only results for $\kzipf=0$ and $\kzipf=1$ for \covid19.
% For \citibike, where the query pool is already very small, we evaluate only for $\kzipf=0$ to not reduce it even more with skewed sampling.

% \heading{Metrics.}
% $\bullet$ {\em Cumulative budget}: the average budget consumed across all the database partitions.
% $\bullet$ {\em Systems metrics:} runtime, DRAM consumption.
% $\bullet$ {\em \Empiricalconvergence}: We periodically evaluate the quality of \sysname's histogram by running a validation workload sampled from the same query pool. We measure the accuracy of the histogram as the fraction of queries that are answered with error $\ge \alpha/2$ by the histogram. We define {\em \empiricalconvergence} as the number of histogram updates necessary to reach 90\% validation accuracy.

% \subsection{Use Case (1): \Nonpartitioneddb}
% \label{sec:evaluation:non-partitioned-database}

% \begin{figure*}[tp]
%     \subfigure{
%         \includegraphics[width=0.5\textwidth]{results/monoblock/covid19/laplace_vs_hybrid/cumulative_budget_utilization_legend.pdf}
%     }
%     \setcounter{subfigure}{0}
%     \\ \vspace{-0.5cm}
%     \subfigure[\sysname on \covid19 $\kzipf=0$]{
%         \includegraphics[width=0.23\textwidth]{results/monoblock/covid19/laplace_vs_hybrid/cumulative_budget_utilization_zipf0.pdf}
%         \label{fig:monoblock_covid_system_eval_zipf0}
%     }
%     \hfill
%     \subfigure[\sysname on \covid19 $\kzipf=1$]{
%         \includegraphics[width=0.23\textwidth]{results/monoblock/covid19/laplace_vs_hybrid/cumulative_budget_utilization_zipf1.pdf}
%         \label{fig:monoblock_covid_system_eval_zipf1}
%     }
%     \hfill
%     \subfigure[\sysname on \citibike $\kzipf=0$]{
%         \includegraphics[width=0.23\linewidth]{results/monoblock/citibike/laplace_vs_hybrid/cumulative_budget_utilization_zipf0.pdf}
%         \label{fig:monoblock_citibike_system_eval_zipf0}
%     }
%     \subfigure[\Empiricalconvergence]{
%         \includegraphics[width=0.23\linewidth]{results/monoblock/covid19/convergence/lr_convergence_updates.pdf}
%         \label{fig:monoblock_covid_empirical_convergence}
%     }
%     \caption{\small {\bf \Nonpartitioneddb: (a-c) system-wide evaluation (Question 1); (d) \empiricalconvergence for \pmwbypass vs. \pmw (Question 2).} (a-c) \sysname is instantiated with one \pmwbypass and \exactcache. Across all three workloads, \sysname significantly improves budget consumption compared to both its baselines. (d) Uses \covid19 $\kzipf=1$. \pmwbypass has similar \empiricalconvergence to \pmw, and both converge faster with much larger $\lr$ (e.g., $\lr=0.2$) than anticipated by \theoreticalconvergence ($0.00625$ here). \kelly{The Y axis legend in (d) overrides the Y axis labels}
%     }
%     \label{fig:monoblock_eval}
% \end{figure*}

% \heading{System-wide evaluation.} {\em Question 1: In a non-partitioned static database, does \sysname significantly improve privacy budget consumption compared to vanilla PMW and a simple \exactcache?}
% \F\ref{fig:monoblock_covid_system_eval_zipf0}-\ref{fig:monoblock_citibike_system_eval_zipf0} show the cumulative privacy budget consumed as the workload progresses to $70K$ queries for three workloads.
% Two workloads are for \covid19 -- one uniform ($\kzipf=0$) and one skewed ($\kzipf=1$) -- and one uniform workload for \citibike.
% Across all three workloads, \sysname clearly outperforms both baselines.
% The benefit is enormous compared to vanilla \pmw: XX-33.2$\times$! Although \pmw converges fast, it spends significant privacy in doing so.  \sysname instead spends little during training and then gets query results for free.
% Compared to the \exactcache, the benefit is less dramatic, but still significant.
% On the uniform \covid19 workload (\F\ref{fig:monoblock_covid_system_eval_zipf0}), the improvement over \exactcache is the greatest: XX$\times$.  There, queries are fairly unique, so the \exactcache has low hit rate.
% On the skewed workload (\F\ref{fig:monoblock_covid_system_eval_zipf1}), queries are less diverse and the \exactcache's hit rate is higher.
% This results leave less room for improvement for \sysname: XX$\times$ better than \exactcache.
% For \citibike (\F\ref{fig:monoblock_citibike_system_eval_zipf0}), whose query pool is much smaller ($2K$ unique queries), there is significant exact repetition. % even for a uniform workload with $70K$ total queries. 
% Still, even in this case, \sysname exhibits a 1.54$\times$ improvement over the \exactcache baseline, and compared to the PMW baseline (not shown in that figure for visualization reasons), \sysname is $33.2\times$ better!
% Thus, \sysname as a whole {\em significantly improves privacy budget consumption in non-partitioned databases} (goal (G5)).

% \begin{figure}[t]
%     \centering
%     \subfigure[Impact of heuristic parameter $C_0$]{
%         \includegraphics[width=0.47\linewidth]{results/monoblock/covid19/heuristics/cumulative_budget_utilization_zipf1.pdf}
%         \label{fig:monoblock_covid_heuristics}
%     }
%     \subfigure[Impact of parameter $\lr$]{
%         \includegraphics[width=0.47\linewidth]{results/monoblock/covid19/learning_rates/cumulative_budget_utilization_zipf1.pdf}
%         \label{fig:monoblock_covid_learning_rates}
%     }
%     \caption{ \small {\bf Impact of major parameters on \pmwbypass performance (Question 3).} Uses \covid19 $\kzipf=1$.
%         Being too optimistic or pessimistic about the histogram's state (a), or too aggressive or timid in learning from each update (b), give poor performance.  However, good values for $C_0$ and $\lr$ give good performance. \kelly{the legend text in (a) is cut}
%     } \label{fig:pmwbypass_params_eval}
% \end{figure}

% \heading{\pmwbypass evaluation.}
% Using \covid19 $\kzipf=1$, we microbenchmark \pmwbypass to understand the behavior of this key \sysname component.
%     %
%     {\em Question 2: Does \pmwbypass converge similarly to \pmw in practice?}
% Theoretically, we have shown that \pmwbypass enjoys similar \theoreticalconvergence to \pmw, albeit with degraded parameters (\S\ref{sec:pmw-bypass}, Guarantees).
% \F\ref{fig:monoblock_covid_empirical_convergence} compares {\em \empiricalconvergence} (defined in \S\ref{sec:evaluation:methodology}, Metrics) of \pmwbypass vs. \pmw, as a function of the main parameter impacting convergence speed: the learning rate $\lr$.
% We make three observations, the first two in which theory and practice agree, the last in which they differ.
% First, the results confirm the theory that (1) \pmwbypass and \pmw converge similarly but (2) for ``good'' values of $\lr$, vanilla \pmw converges a bit faster: e.g, for $\lr=0.2$, \pmwbypass needs XX updates to converge while \pmw needs XX.
% Second, as theory suggests, very large values of $\lr$ (e.g., $\lr \ge 1$ for \pmwbypass and $\lr \ge 3$ for \pmw) impede convergence in practice as well.
% Third, while theoretically it can be shown that setting $\lr=\alpha/8=0.065$ is optimal for \theoreticalconvergence -- and indeed this value is typically hard-coded in PMW protocols~\cite{complexity} -- we find that empirically, {\em much larger} values of $\lr$ (such as $\lr=0.2$, so $40\times$ larger) result in substantially fewer queries needed to converge.
% This is true for both \pmw and \pmwbypass, and for other datasets and workloads.
% This justifies our urge to take into account empirical behavior when analyzing and tuning mechanisms (goal (G4)).

%     {\em Question 3: How do the \pmwbypass parameters impact privacy budget consumption?}
% We experimented with all parameters of the preceding mechanisms ($C_0$, $S_0$, $\lr$, $\tau$, and $\gamma$) and found that the two most impactful in practice are: (a) $C_0$, the heuristic's initial threshold for the number of updates each bin involved in a query must have received in order to invoke the histogram for that query; and (b) $\lr$, the learning rate.
% \F\ref{fig:pmwbypass_params_eval} shows the results.
%     {\em Heuristic $C_0$ (\F\ref{fig:monoblock_covid_heuristics}):} Higher $C_0$ means more pessimistic assessment of histogram readiness.  If $C_0$ is too high ($C_0=10K$ updates) \pmwbypass never uses the \pmw, hence mimicking an \exactcache.  When $C_0$ is too low ($C_0=1$ update) \pmwbypass overpays for the histogram's training.  A good value is $C_0=100$ updates, for which we found that $S_0=5$ works well for our workloads.
%     {\em Learning rate $\lr$ (\F\ref{fig:monoblock_covid_learning_rates}):}
% Higher $\text{lr}$ means more aggressive learning from each (external) update.
% Both too aggressive ($\text{lr}=1$) and too timid ($\text{lr}=0.05$) learning from each update prevent fast convergence of the histogram; good values hover around $\text{lr}=0.2$.
% Overall, we find that few hyper-parameters in \pmwbypass impact performance, and even for those, performance is fairly stable around ``good values,'' making these parameters easy to tune (goal (G7)).


% \subsection{Use Case (2): Partitioned Static Database}
% \label{sec:evaluation:partitioned-static-database}

% \begin{figure*}[tp]
%     \centering
%     \subfigure{
%         \includegraphics[width=0.5\textwidth]{results/multiblock/static/covid19/laplace_vs_hybrid/cumulative_budget_utilization_legend.pdf}
%     }
%     \setcounter{subfigure}{0}
%     \\ \vspace{-0.5cm}
%     \subfigure[\sysname on \covid19 $\kzipf=0$]{
%         \includegraphics[width=0.23\textwidth]{results/multiblock/static/covid19/laplace_vs_hybrid/cumulative_budget_utilization_zipf0.pdf}
%         \label{fig:multiblock_static_covid_cumulative_budget_consumption_zipf0}
%     }
%     \hfill
%     \subfigure[\sysname on \covid19 $\kzipf=1$]{
%         \includegraphics[width=0.23\textwidth]{results/multiblock/static/covid19/laplace_vs_hybrid/cumulative_budget_utilization_zipf1.pdf}
%         \label{fig:multiblock_static_covid_cumulative_budget_consumption_zipf1}
%     }
%     \hfill
%     \subfigure[\sysname on \citibike $\kzipf=0$]{
%         \includegraphics[width=0.23\textwidth]{results/multiblock/static/citibike/laplace_vs_hybrid/cumulative_budget_utilization_zipf0.pdf}
%         \label{fig:multiblock_static_citibike_cumulative_budget_consumption_zipf0}
%     }
%     \hfill
%     \subfigure[Tree structure evaluation]{
%         \includegraphics[width=0.23\textwidth]{results/multiblock/static/covid19/tree/tree_vs_linear_zipf1.pdf}
%         \label{fig:tree_vs_linear}
%     }
%     \caption{\small {\bf \Partitionedstaticdb: (a-c) system-wide evaluation (Question 4); (d) \pmwbypasstree vs. one-histogram-per-partition baseline (Question 5).}
%         (a-c) \sysname is instantiated with a tree-structured \pmwbypass and \exactcache.
%         Across all workloads, \sysname significantly improves budget consumption compared to both a single \exactcache and a tree-structured set of Exact-Caches.
%         (d) Uses \covid19 $\kzipf=1$. Compared with a flat structure, the tree structure for histograms is beneficial when queries request more partitions.
%     }
%     \label{fig:multiblock_static_eval}
% \end{figure*}

% We now examine the static timeseries use case, where most queries request data by time ranges, accessing a subset of the database. We split the static database into 50 partitions. Each query in the workload is run on a randomly-selected window of 1--50 partitions.  \todostudents{Do we select \# of partitions uniformly?}

% \heading{System-wide evaluation.}  {\em Question 4: In a partitioned static database, does \sysname significantly improve privacy budget consumption, compared to a single \exactcache and a tree-structured set of Exact-Caches?}
% \F\ref{fig:multiblock_static_covid_cumulative_budget_consumption_zipf0}-\ref{fig:multiblock_static_citibike_cumulative_budget_consumption_zipf0} show the average consumed budget across the partitions, as the workloads advance up to $300K$ queries.
% Compared to the static use case, the system can now support many more queries under the fixed $\epsilon_G=10$-DP guarantee, because each query now consumes privacy only from the accessed partitions (the benefit of query splitting and parallel composition).
% The results show that \sysname improves privacy budget consumption by \partitionedstaticdbimprovement compared to the best-performing baseline for each workload.
% Interestingly, applying the tree structure that works for PMW to the \exactcache, i.e., having multiple \exactcaches organized in a binary tree, does not always outperform the simple \exactcache, specifically for the \covid19 $\kzipf=0$ workload.
% For this workload, there is such a large variety of unique queries that the hit rate for both caches is low.
% The tree-structured \exactcache fragments the query workload among cache nodes, lowering the hit rate even further.
% For workloads with higher query repetition (\covid19 and \citibike $\kzipf=1$), the hit rate is higher and the tree starts to help.

% \heading{\bf \Pmwbypasstree evaluation.}
% {\em Question 5: When is the tree structure for \pmwbypass histograms beneficial?}
% \F\ref{fig:tree_vs_linear} compares \pmwbypasstree to the baseline design outlined in \S\ref{sec:tree-structured-caching}: maintaining one histogram per partition (hence a linear structure).  No \exactcache is used.
% Here, each query is requesting a window of partitions whose size is sampled from a Gaussian distribution with std-dev $5$ and mean ranging from $1-50$ (x-axis).
% Compared to the flat structure, the tree structure for histograms is beneficial when queries tend to request more partitions: over 20 in this experiment.
% Because the tree maintains more histograms than the flat structure, it fragments the query workload more, so each histogram is updated more slowly and direct-Laplace is used more.
% When queries request larger windows of partitions, the tree's advantage to combine fewer results makes up for this privacy overhead caused by histogram maintenance.
% When queries request smaller windows of partitions, the histogram management overhead dominates and the linear structure is more beneficial.
% \asaf{This graph is a bit noisy -- someone may wonder why the green line moves up and down so much. We could just summarize the results here by saying the tree structure is beneficial when there are more than 20 queries, for more details see graph in appendix, since the actual graph is confusing / doesn't add much information}

% \subsection{Use Case (3): Partitioned Streaming Database}
% \label{sec:evaluation:partitioned-streaming-database}

% \begin{figure*}[tp]
%     \centering
%     \subfigure{
%         \includegraphics[width=0.5\textwidth]{results/multiblock/streaming/covid19/laplace_vs_hybrid/cumulative_budget_utilization_legend.pdf}
%     }
%     \setcounter{subfigure}{0}
%     \\ \vspace{-0.5cm}
%     \subfigure[\sysname on \covid19 $\kzipf=0$]{
%         \includegraphics[width=0.23\textwidth]{results/multiblock/streaming/covid19/laplace_vs_hybrid/cumulative_budget_utilization_zipf0.pdf}
%         \label{fig:multiblock_streaming_covid_cumulative_budget_consumption_zipf0}
%     }
%     \hfill
%     \subfigure[\sysname on \covid19 $\kzipf=1$]{
%         \includegraphics[width=0.23\textwidth]{results/multiblock/streaming/covid19/laplace_vs_hybrid/cumulative_budget_utilization_zipf1.pdf}
%         \label{fig:multiblock_streaming_covid_cumulative_budget_consumption_zipf1}
%     }
%     \hfill
%     \subfigure[\sysname on \citibike $\kzipf=0$]{
%         \includegraphics[width=0.23\textwidth]{results/multiblock/streaming/citibike/laplace_vs_hybrid/cumulative_budget_utilization_zipf0.pdf}
%         \label{fig:multiblock_streaming_citibike_cumulative_budget_consumption_zipf0}
%     }
%     \hfill
%     \subfigure[Runtime evaluation \kelly{Not ready yet! I will update this.}]{
%         \includegraphics[width=0.23\textwidth]{results/multiblock/streaming/syseval/runtime.pdf}
%         \label{fig:runtime_eval}
%     }
%     \caption{\small {\bf \Partitionedstreamingdb: (a-c) system-wide consumed budget evaluation (Question 6); (d) runtime evaluation (Question 7).}
%         (a-c) \sysname is instantiated with a tree-structured \pmwbypass, \exactcache, with and without warmup.
%         Across all workloads, \sysname significantly improves budget consumption compared to the baselines, especially when warmup is enabled.
%         (d) Uses \covid19 $\kzipf=1$. XXX.
%     }
%     \label{fig:multiblock_streaming_system_eval}
% \end{figure*}

% \heading{System-wide evaluation.}  {\em Question 6: In streaming databases partitioned by time, does \sysname significantly improve privacy budget consumption compared to a single \exactcache and a tree-structured set of Exact-Match Caches?  Does warmup help?}
% \F\ref{fig:multiblock_streaming_covid_cumulative_budget_consumption_zipf0}-\ref{fig:multiblock_streaming_citibike_cumulative_budget_consumption_zipf0} shows privacy budget consumption of \sysname compared to these baselines.
% In these experiments, partitions are not all available upfront, but arrive over time, and the queries are set to request the latest $P$ partitions, with $P$ chosen uniformly at random between $1$ and the number of available partitions.
% \todostudents{Why do the lines keep going up?}
% Across all workloads, \sysname improves budget performance significantly across both baselines, especially when warmup is enabled.
% Without warmup, the benefit at the end of the workload is at least XX-XX$\times$.
% Warmup gives \partitionedstreamingdbimprovement improvement over the best-performing baseline in each of our three workloads.

% \subsection{Runtime and Memory Evaluation}
% \label{sec:evaluation:runtime-memory}
% \begin{table}
%     \footnotesize
%     \centering
%     \begin{tabular}{|l|l|}
%         \hline
%         {\bf Dataset}           & {\bf \sysname memory usage} \\
%         \hline
%         {\bf \covid19 (Zipf 0)} & 5.21 MB                     \\
%         \hline
%         {\bf \covid19 (Zipf 1)} & 4.04 MB                     \\
%         \hline
%         {\bf \citibike}         & 1.43 GB                     \\
%         \hline
%     \end{tabular}
%     \vspace{0.35cm}
%     \caption{{\small {\bf Redis Memory Usage.} \kelly{Not Ready I will update this.}}}
%     \label{tab:datasets}
% \end{table}

% {\em Question 7: How does runtime of \sysname compare to XX, and how is it split among its major components?}
% \F\ref{fig:runtime_eval} shows...

% \asaf{We should say somewhere (maybe here) that we don't actually have to store Turbo's data structures fully in memory}

% {\em Question 8: What is \sysname's memory consumption?} XXX.


==> sections/motivation.tex <==
\section{DPF and Its Limitations}
\label{sec:motivation}
